Presynthesis: Towards Scaling Up Program Synthesis with Finer-Grained Abstract Semantics

Abstract semantics has proven to be instrumental for accelerating search-based program synthesis, by enabling the sound pruning of a set of incorrect programs (without enumerating them). One may expect faster synthesis with increasingly finer-grained abstract semantics. Unfortunately, to the best of our knowledge, this is not the case, yet. The reason is because, as abstraction granularity increases -- while fewer programs are enumerated -- pruning becomes more costly. This imposes a fundamental limit on the overall synthesis performance, which we aim to address in this work. Our key idea is to introduce an offline presynthesis phase, which consists of two steps. Given a DSL with abstract semantics, the first semantics modeling step constructs a tree automaton A for a space of inputs -- such that, for any program P and for any considered input I, A has a run that corresponds to P's execution on I under abstract semantics. Then, the second step builds an oracle O for A. This O enables fast pruning during synthesis, by allowing us to efficiently find exactly those DSL programs that satisfy a given input-output example under abstract semantics. We have implemented this presynthesis-based synthesis paradigm in a framework, Foresighter. On top of it, we have developed three instantiations for SQL, string transformation, and matrix manipulation. All of them significantly outperform prior work in the respective domains.

==> eval-figures/RQ2-table.tex <==
\begin{table}
\footnotesize
\begin{tabular}{lrrrrr}
\toprule
\multirow{2}{*}{\textbf{Tool}} & \multirow{2}{*}{\textbf{\#Solved}} & \multicolumn{2}{c}{\textbf{Speed up}} & \multicolumn{2}{c}{\textbf{Solving time}}\\
                      &                           & Median & Geomean             &  Median & Avg.\\
\midrule
$\tool$ & 2,603 & 1x & 1x & 0.01s & 21.8s \\
$\cubesdc$ & 2,564 & 129.5x & 41.6x & 1.6s & 15.6s \\ 
$\cubes$ & 2,274 & 92.1x & 51.2x & 1.78s & 31.0s \\
$\patsql$ & 1,951 & 0.9x & 0.7x & 0.06s & 6.2s \\
$\blazesql$ & 1,738 & 118.5x & 126.5x & 0.58s  & 11.8s\\
\bottomrule
\end{tabular}

\caption{ Summary of coverage and speedup. Speedup is calculated using on benchmarks solved by both $\tool$ and the given baseline. Solving time is calculated on all solved benchmarks by a given tool.}
\label{fig:RQ2:table}
\end{table}

==> figures/fta-construction-rules.tex <==
\begin{figure}[!t]
%\scriptsize
%\footnotesize
\small 
\centering
\[
\arraycolsep=3pt\def\arraystretch{1}
\begin{array}{l}
    \hfill
\textsc{(Offline-Var)}~
\ 
\irule{
\variablesymbol  \in \allvariablesymbols
\quad 
s \rightarrow x \in R 
\quad
\graybox{$\abstractvalue \in \mathcal D_x$} 
}{
\ftastate_{s}^\abstractvalue \in \ftastates 
\quad 
\variablesymbol \in \ftaalphabet
\quad 
\variablesymbol \ftatransitionarrow \ftastate_{s}^\abstractvalue \in \ftatransitions
}
\qquad \quad 
\textsc{(Offline-Final)}~
\ 
\irule{
\ftastate_{\startsymbol}^{\abstractvalue} \in \ftastates
\quad 
\graybox{$\gamma(\abstractvalue) \neq \emptyset$}
}{
\ftastate_{\startsymbol}^{\abstractvalue} \in \ftafinalstates
}
\hfill 

\\ \\ 

\hfill
\textsc{(Offline-Prod)}~
\ 
\irule{
%f \in \terminalsymbols \setminus \allvariablesymbols
%\quad 
\grammarsymbol \productionarrow \dsloperator( \grammarsymbol_1, \mydots, \grammarsymbol_n ) \in \productions
\quad 
\ftastate_{\grammarsymbol_i}^{\abstractvalue_i} \in \ftastates
\quad 
\abstractvalue = 
\transformer{f}(\abstractvalue_1, \mydots, \abstractvalue_n) 
}{
\ftastate_{\grammarsymbol}^\abstractvalue \in \ftastates 
\quad
\dsloperator \in \ftaalphabet
\quad 

\dsloperator\!\left( \ftastate_{\grammarsymbol_1}^{\abstractvalue_i}, \mydots, \ftastate_{\grammarsymbol_n}^{\abstractvalue_n} \right) \ftatransitionarrow \ftastate_{\grammarsymbol}^{\abstractvalue} \in \ftatransitions
}
\hfill

\end{array}
\]
\caption{The rules for constructing the offline FTA $\fta = ( \ftastates, \ftaalphabet, \ftafinalstates, \ftatransitions)$, i.e., \buildftaalg~in \algorithmref{alg:top-level}, given a grammar $\grammar = ( \terminalsymbols, \nonterminalsymbols, \productions, \startsymbol )$ and an abstract transformer $\transformer{\cdot}$. Here, $\abstractdomain_{x}$ denotes the domain of abstract values for variable $x$, and we highlight the difference between these rules and their counterparts in \autoref{fig:prior-fta-construction-rules} as \graybox{gray}.}
\label{fig:fta-construction-rules}
\end{figure}


\endinput

\begin{figure}[!t]
%\scriptsize
%\footnotesize
\small 
\centering

\[
\arraycolsep=3pt\def\arraystretch{1}
\begin{array}{l}


\text{[Var]}
\ 
\irule{
\variablesymbol  \in \allvariablesymbols
\quad
\boxed{ \abstractvalue \in \abstractdomain_{\variablesymbol} }
}{
\ftastate_{\variablesymbol}^{\abstractvalue} \in \ftastates 
\quad 
\variablesymbol \in \ftaalphabet
\quad 
\variablesymbol \ftatransitionarrow \ftastate_{\variablesymbol}^{\abstractvalue}
}

\quad 



\text{[Const]}
\ 
\irule{
\constantsymbol  \in \allconstantsymbols
\quad
\abstractvalue = \abstractionfunction^{\abstractdomain} \big( \constantsymbol = \concretetransformer{\constantsymbol} \big)
}{
\ftastate_{\constantsymbol}^{\abstractvalue} \in \ftastates 
\quad 
\constantsymbol \in \ftaalphabet
\quad 
\constantsymbol \ftatransitionarrow \ftastate_{\constantsymbol}^{\abstractvalue}
}



\\ \\ 


\text{[Prod]}
\ 
\irule{
\big( \grammarsymbol \productionarrow \dsloperator( \grammarsymbol_1, \mydots, \grammarsymbol_n ) \big) \in \productions
\quad 
\ftastate_{\grammarsymbol_i}^{\abstractvalue_i} \in \ftastates
\quad 
\abstractvalue = 
\abstractionfunction^{\abstractdomain}
\big(
\abstracttransformer{\dsloperator} 
( \abstractvalue_1, \mydots, \abstractvalue_n ) 
\big)
}{
\ftastate_{\grammarsymbol}^{\abstractvalue} \in \ftastates 
\quad
\dsloperator \in \ftaalphabet
\quad 
\big( 
\dsloperator( \ftastate_{\grammarsymbol_1}^{\abstractvalue_1}, \mydots, \ftastate_{\grammarsymbol_n}^{\abstractvalue_n} ) \ftatransitionarrow \ftastate_{\grammarsymbol}^{\abstractvalue} \big) \in \ftatransitions
}


\quad


\text{[Final]}
\ 
\irule{
\boxed{ \ftastate_{\startsymbol}^{\abstractvalue} \in \ftastates } 
}{
\ftastate_{\startsymbol}^{\abstractvalue} \in \ftafinalstates
}



\end{array}
\]

\caption{Rules for constructing FTA $\fta = ( \ftastates, \ftaalphabet, \ftafinalstates, \ftatransitions)$, given a DSL with grammar $\grammar = ( \terminalsymbols, \nonterminalsymbols, \productions, \startsymbol )$ and abstract transformers $\abstracttransformername$. 
$\abstractdomain_{\grammarsymbol}$ denotes the domain of abstract values for grammar symbol $\grammarsymbol$.}
\label{fig:fta-construction-rules}
\end{figure}



==> figures/online-slicing-rules.tex <==
%\newcommand{\oracleCheck}[3]{#1 \models #2 \nearrow #3}
%\newcommand{\oracleCheck}[3]{#1 \models #2 \rightsquigarrow #3}
%\newcommand{\slicingstates}{\ftastates^{\mathcal S}}
\begin{figure}[!t]
%\scriptsize
%\footnotesize
\small 

\centering
\[
\arraycolsep=3pt\def\arraystretch{1}
\begin{array}{l}

\hfill
\textsc{(Online-Base)}~
\
\irule{
\outputex \in \gamma(\abstractvalue)
\quad 
q_{\startsymbol}^{\abstractvalue} \in \ftafinalstates
\quad 
\bottomup(q_{\startsymbol}^\abstractvalue, \inputex)
}{
q_{\startsymbol}^{\abstractvalue} \in \ftastates'
\quad 
q_{\startsymbol}^{\abstractvalue} \in \ftafinalstates'
} 
\hfill

\\
\\

\hfill
\textsc{(Online-Rec)}~
\ 
\irule{
\dsloperator\!\left( q_1, \dots, q_n \right) \ftatransitionarrow \ftastate \in \ftatransitions
\quad 
q \in \ftastates'
\quad 
\bottomup(q_i, \inputex)
}{
q_1, \dots q_n \in \ftastates'
\quad 
\dsloperator\!\left( q_1, \dots, q_n \right) \ftatransitionarrow \ftastate \in \ftatransitions'
}
\hfill
\end{array}
\]

\caption{Rules for extracting the slice $\ftaslice = (\ftastates', \ftaalphabet, \ftafinalstates', \ftatransitions')$ for the offline FTA $\fta = (\ftastates, \ftaalphabet, \ftafinalstates, \ftatransitions)$ and the IO example $e$. The predicate $\bottomup$ checks the bottom-up condition in \lemmaref{lemma:slice-condition}.} 
\label{fig:online-slicing-rules}
\end{figure}


==> figures/slicing-oracle-rules.tex <==
\begin{figure}[!t]
%\scriptsize
%\footnotesize
\small 
\centering

\begin{gather*}
    \forall q_{s}^{\abstractvalue} \in Q.\quad \slicingoracle\left[q_{s}^{\abstractvalue}\right] \coloneqq \lambda \inputex. \bigvee_{\ftatransition \in \ftatransitions[q_s^{\abstractvalue}]} \left\{
    \begin{array}{lllc}
        a = \alpha(\inputex(x)) & & \textbf{if}\ \ \ftatransition = x \rightarrow q_{s}^{\abstractvalue} & \textsc{(Oracle-Base)}\\ 
        \wedge_{i=1}^n \mathcal O[q_i](\inputex) & & \textbf{if}\ \ \ftatransition = \dsloperator\!\left(q_1, \mydots, q_n\right) \ftatransitionarrow q_{s}^{\abstractvalue} & \textsc{(Oracle-Rec)}\\
    \end{array}
    \right.
\end{gather*}
\vspace{-0.5em}
\caption{Rules for constructing the \soname $\slicingoracle$ for an offline FTA $\fta = ( \ftastates, \ftaalphabet, \ftafinalstates, \ftatransitions)$, where $\slicingoracle[q]$ denotes the predicate assigned to state $q$, and $\ftatransitions[q]$ denotes the subset of transitions whose outcome is $q$.}
\label{fig:slicing-oracle-rules}
\end{figure}

\endinput

\begin{figure}[!t]
%\scriptsize
%\footnotesize
\small 
\centering


\[
\arraycolsep=3pt\def\arraystretch{1}
\begin{array}{l}

\hfill
\textsc{(Oracle-Var)}~
\
\irule{
\variablesymbol  \in \allvariablesymbols
\quad
x \rightarrow \ftastate_{\variablesymbol}^\abstractvalue \in \ftatransitions
%\ftastate_{\variablesymbol}^v \in \ftastates 
%\quad 
%O[x'] = \left\{ 
%\begin{aligned}
%v & & x' = x \\
%\top & & x' \neq x
%\end{aligned}
%\right.
%O = \big\{x' \mapsto \textbf{ite}(x = x', v, \top)\quad \textbf{for}~x' \in \allvariablesymbols\big\}
}{
\big\{x' \mapsto \textbf{ite}(x = x', \abstractvalue, \top)~\big|~x' \in \allvariablesymbols\big\} \in \mathcal \slicingoracle[\ftastate_{\variablesymbol}^\abstractvalue]
} 

\\
\\

\hfill
\textsc{(Oracle-Prod)}~
\ 
\irule{
\dsloperator\!\left( \ftastate_{\grammarsymbol_1}^{\abstractvalue_1}, \mydots, \ftastate_{\grammarsymbol_n}^{\abstractvalue_n} \right) \ftatransitionarrow \ftastate_{\grammarsymbol}^{\abstractvalue} \in \ftatransitions
\quad 
O_i \in \slicingoracle[\ftastate_{\grammarsymbol_i}^{\abstractvalue_i}]
}{
\left\{x \mapsto \bigsqcap_{i=1}^n O_i(x) ~\big|~ x \in \allvariablesymbols\right\} \in \slicingoracle[\ftastate_{\grammarsymbol}^\abstractvalue]
}
\hfill
\end{array}
\]

\caption{Rules for constructing an \soname $\slicingoracle$, given an offline AFTA $\fta = ( \ftastates, \ftaalphabet, \ftafinalstates, \ftatransitions)$.}
\label{fig:slicing-oracle-rules}
\end{figure}


==> figures/top-level-algs.tex <==


\begin{figure}[!t]
\small 
\begin{algorithm}[H]
\caption{Presynthesis and synthesis algorithms.}
\label{alg:top-level}
\begin{algorithmic}[1]

\Statex\myprocedure{\presynthesisalg($\grammar$)}
\vspace{1pt}

\Statex\myinput{$\grammar$ is a context-free grammar that is associated with abstract semantics.}

\Statex\Output{An AFTA $\fta$ and a slicing oracle $\slicingoracle$.} \ruyi{we don't need to distinguish between AFTA and FTA, do we?}
\vspace{2pt}



\State 
$\fta \assign \buildftaalg( \grammar )$;

\State 
$\slicingoracle \assign \buildslicingoraclealg( \fta )$;



\State 
\Return $( \fta, \slicingoracle )$;



\vspace{5pt}


\Statex\myprocedure{\synthesisalg($\ioexs, \fta, \slicingoracle$)}
\vspace{1pt}

\Statex\myinput{$\ioexs = \{ \ioex_1, \mydots, \ioex_n \}$ is a set of $n$ input-output examples.} 

\Statex\myinput{$\fta$ and $\slicingoracle$ are the pre-synthesized FTA and slicing oracle.}

\Statex\Output{A program $\prog$ that satisfies $\ioexs$, or $\mynull$ indicating no such program is found.}
\vspace{2pt}


\State
$\ftaslice \assign \slicealg( \fta, \ioex_1, \slicingoracle )$;

\State 
$\prog \assign \searchalg( \ftaslice, \ioexs )$;

\State
\Return $\prog$;


\end{algorithmic}
\end{algorithm}
\end{figure}



